Adaptive Sampling for Stochastic Risk-Averse Learning

In high-stakes machine learning applications, it is crucial to not only perform well on average, but also when restricted to difficult examples. To address this, we consider the problem of training models in a risk-averse manner. We propose an adaptive sampling algorithm for stochastically optimizing the Conditional Value-at-Risk (CVaR) of a loss distribution, which measures its performance on the $\alpha$ fraction of most difficult examples. We use a distributionally robust formulation of the CVaR to phrase the problem as a zero-sum game between two players, and solve it efficiently using regret minimization. Our approach relies on sampling from structured Determinantal Point Processes (DPPs), which enables scaling it to large data sets. Finally, we empirically demonstrate its effectiveness on large-scale convex and non-convex learning tasks.

==> sections/tables/both_.tex <==
\begin{table}
\scriptsize
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.25}
\caption{
Test accuracy/loss (mean $\pm$ s.d.) over five independent data splits with
both distribution shift 
with no resampling
In shaded bold we indicate the best algorithms.}
\label{table:both:}
\begin{tabular}{cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c|}{Data Set} &  \multicolumn{2}{c|}{\adacvar}  & \multicolumn{2}{c|}{\trunkcvar}  & \multicolumn{2}{c|}{\softcvar} & \multicolumn{2}{c}{\mean}  \\
\midrule \multirow{8}{*}{\STAB{\rotatebox[origin=c]{90}{Train Set Shift}}\hspace{-5mm}}
& Adult      &  0.59 $\pm$ 0.0 & 0.66 $\pm$ 0.0 &  0.48 $\pm$ 0.1 & 0.69 $\pm$ 0.0 &  0.51 $\pm$ 0.0 & 1.14 $\pm$ 0.0 &  0.46 $\pm$ 0.0 & 1.25 $\pm$ 0.0 \\
& Australian &  0.48 $\pm$ 0.1 & 0.73 $\pm$ 0.1 &  0.33 $\pm$ 0.1 & 0.75 $\pm$ 0.0 &  0.14 $\pm$ 0.0 & 1.38 $\pm$ 0.1 &  0.10 $\pm$ 0.0 & 1.30 $\pm$ 0.1 \\
& German     &  0.27 $\pm$ 0.1 & 0.86 $\pm$ 0.0 &  0.37 $\pm$ 0.1 & 0.79 $\pm$ 0.1 &  0.29 $\pm$ 0.0 & 1.26 $\pm$ 0.1 &  0.37 $\pm$ 0.1 & 0.91 $\pm$ 0.1 \\
& Monks      &  0.10 $\pm$ 0.0 & 0.92 $\pm$ 0.1 &  0.28 $\pm$ 0.1 & 0.76 $\pm$ 0.0 &  0.10 $\pm$ 0.0 & 2.01 $\pm$ 0.1 &  0.10 $\pm$ 0.0 & 1.25 $\pm$ 0.1 \\
& Phoneme    &  0.48 $\pm$ 0.2 & 0.71 $\pm$ 0.0 &  0.41 $\pm$ 0.1 & 0.69 $\pm$ 0.0 &  0.33 $\pm$ 0.0 & 1.51 $\pm$ 0.0 &  0.40 $\pm$ 0.1 & 1.23 $\pm$ 0.1 \\
& Spambase   &  0.69 $\pm$ 0.0 & 0.58 $\pm$ 0.0 &  0.63 $\pm$ 0.0 & 0.61 $\pm$ 0.0 &  0.54 $\pm$ 0.0 & 0.84 $\pm$ 0.1 &  0.50 $\pm$ 0.0 & 0.81 $\pm$ 0.0 \\
& Splice     &  0.72 $\pm$ 0.0 & 0.56 $\pm$ 0.0 &  0.69 $\pm$ 0.0 & 0.64 $\pm$ 0.0 &  0.56 $\pm$ 0.0 & 0.80 $\pm$ 0.0 &  0.10 $\pm$ 0.0 & 1.35 $\pm$ 0.0 \\
& Titanic    &  0.31 $\pm$ 0.3 & 0.78 $\pm$ 0.1 &  0.50 $\pm$ 0.4 & 0.70 $\pm$ 0.0 &  0.09 $\pm$ 0.0 & 1.67 $\pm$ 0.1 &  0.09 $\pm$ 0.0 & 1.12 $\pm$ 0.2 \\
\bottomrule
\end{tabular}
\end{table}


==> sections/tables/both_upsample.tex <==
\begin{table}
\scriptsize
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.25}
\caption{
Test accuracy/loss (mean $\pm$ s.d.) over five independent data splits with
both distribution shift 
with upsampling
In shaded bold we indicate the best algorithms.}
\label{table:both:upsample}
\begin{tabular}{cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c|}{Data Set} &  \multicolumn{2}{c|}{\adacvar}  & \multicolumn{2}{c|}{\trunkcvar}  & \multicolumn{2}{c|}{\softcvar} & \multicolumn{2}{c}{\mean}  \\
\midrule \multirow{8}{*}{\STAB{\rotatebox[origin=c]{90}{Train Set Shift}}\hspace{-5mm}}
& Adult      &  0.56 $\pm$ 0.0 & 0.67 $\pm$ 0.0 &  0.61 $\pm$ 0.2 & 0.69 $\pm$ 0.0 &  0.65 $\pm$ 0.2 & 0.78 $\pm$ 0.4 &  0.62 $\pm$ 0.2 & 0.83 $\pm$ 0.4 \\
& Australian &  0.71 $\pm$ 0.1 & 0.63 $\pm$ 0.0 &  0.42 $\pm$ 0.1 & 0.72 $\pm$ 0.0 &  0.47 $\pm$ 0.3 & 0.93 $\pm$ 0.5 &  0.45 $\pm$ 0.4 & 0.89 $\pm$ 0.4 \\
& German     &  0.52 $\pm$ 0.1 & 0.71 $\pm$ 0.0 &  0.41 $\pm$ 0.1 & 0.76 $\pm$ 0.0 &  0.45 $\pm$ 0.2 & 1.01 $\pm$ 0.3 &  0.47 $\pm$ 0.1 & 0.81 $\pm$ 0.1 \\
& Monks      &  0.58 $\pm$ 0.1 & 0.68 $\pm$ 0.0 &  0.34 $\pm$ 0.1 & 0.74 $\pm$ 0.0 &  0.39 $\pm$ 0.3 & 1.31 $\pm$ 0.7 &  0.35 $\pm$ 0.3 & 0.96 $\pm$ 0.3 \\
& Phoneme    &  0.63 $\pm$ 0.2 & 0.68 $\pm$ 0.0 &  0.57 $\pm$ 0.2 & 0.69 $\pm$ 0.0 &  0.53 $\pm$ 0.2 & 1.02 $\pm$ 0.5 &  0.57 $\pm$ 0.2 & 0.88 $\pm$ 0.4 \\
& Spambase   &  0.77 $\pm$ 0.1 & 0.53 $\pm$ 0.1 &  0.74 $\pm$ 0.1 & 0.61 $\pm$ 0.0 &  0.72 $\pm$ 0.2 & 0.62 $\pm$ 0.2 &  0.70 $\pm$ 0.2 & 0.57 $\pm$ 0.2 \\
& Splice     &  0.84 $\pm$ 0.0 & 0.42 $\pm$ 0.0 &  0.75 $\pm$ 0.1 & 0.59 $\pm$ 0.1 &  0.71 $\pm$ 0.2 & 0.56 $\pm$ 0.3 &  0.50 $\pm$ 0.4 & 0.83 $\pm$ 0.5 \\
& Titanic    &  0.57 $\pm$ 0.4 & 0.70 $\pm$ 0.0 &  0.49 $\pm$ 0.4 & 0.69 $\pm$ 0.0 &  0.48 $\pm$ 0.4 & 1.12 $\pm$ 0.6 &  0.45 $\pm$ 0.4 & 0.85 $\pm$ 0.3 \\
\bottomrule
\end{tabular}
\end{table}

